A stochastic integral of operator-valued functions

In this note we define and study a Hilbert space-valued stochastic integral of operator-valued functions with respect to Hilbert space-valued measures. We show that this integral generalizes the classical Ito stochastic integral of adapted processes with respect to normal martingales and the Ito integral in a Fock space

==> jinfo.tex <==
\jvolume{14}
\jyear{2008}
\jnumber{2}


==> pageinfo.tex <==
\pagespan{11}{22}

